A computational method for the systematic screening of reaction barriers in enzymes: Searching for Bacillus circulans xylanase mutants with greater activity towards a synthetic substrate

We present a semi-empirical (PM6-based) computational method for systematically estimating the effect of all possible single mutants, within a certain radius of the active site, on the barrier height of an enzymatic reaction. The intent of this method is not a quantitative prediction of the barrier heights, but rather to identify promising mutants for further computational or experimental study. The method is applied to identify promising single and double mutants of Bacillus circulans xylanase (BCX) with increased hydrolytic activity for the artificial substrate ortho-nitrophenyl \beta-xylobioside (ONPX$_2$). The estimated reaction barrier for wild-type (WT) BCX is 18.5 kcal/mol, which is in good agreement with the experimental activation free energy value of 17.0 kcal/mol extracted from the observed k$_\text{cat}$ using transition state theory (Joshi et al., Biochemistry 2001, 40, 10115). The PM6 reaction profiles for eight single point mutations are recomputed using FMO-MP2/PCM/6-31G(d) single points. PM6 predicts an increase in barrier height for all eight mutants while FMO predicts an increase for six of the eight mutants. Both methods predict that the largest change in barrier occurs for N35F, where PM6 and FMO predict a 9.0 and 15.8 kcal/mol increase, respectively. We thus conclude that PM6 is sufficiently accurate to identify promising mutants for further study. We prepared a set of all theoretically possible (342) single mutants in which every amino acid of the active site (except for the catalytically active residues E78 and E172) was mutated to every other amino acid. Based on results from the single mutants we construct a set of 111 double mutants consisting of all possible pairs of single mutants with the lowest barrier for a particular position and compute their reaction profile. None of the mutants have, to our knowledge, been prepared experimentally[...].

==> 040-bcx-cosmo-not.tex <==
\section*{Notes}
Joshi, 2000, Table 5: $k_{cat}/K_M$ reported at pH 6 which is not pH optimum of N35D variant, therefore activity of N35D lower than WT.


==> 040-bcx-cosmo-que.tex <==
\section*{Questions}
1) Joshi, 2000: Meaning of \textit{predominant} (Abstract), \textit{apparent} (Abstract), \textit{microscopic} (p. 258) and \textit{major apparent} (Tab. 4a) pKa.\\
2) Joshi, 2000: pKa measurement of N35D reports pKa of D35 to be 3.7.
However, in the crystal structure a strong hydrogen bond between D35 and E172 is observed.
%Is the crystal structure not reporting the most populated protonation state?
%So if in the majority of cases a hydrogen bond is observed, should D35 not be protonated in the majority of cases?
How can a hydrogen bond be observed \textit{in the crystal structure}, when D35 is only protonated in 1\% of the cases?
And therefore, by their own argument, is the pKa of 3.7 correct (structure was solved at pH 7.5)?\\
3) Joshi, 2000: Percentage of correct protonation of D35 reported to be 1\%, but
\[
\mbox{Protonation probability} = \frac{10^{3.7-4.6}}{1+10^{3.7-4.6}} = 0.13
\]
Wrong formula.\\
4) Joshi, 2000: Table 4. How do they know that they have to assign, e.g., the chemical shift of $\delta \Delta = -0.32$ ppm observed in the spectrum of E172 to E78?\\
5) Does a structure resembling the enzyme substrate complex exist?
Is it possible?
6) Assume two carboxylic groups oriented towards each other.
Strong energetic coupling will likely lower the pKa of one and increase the pKa of the other carboxylic group.
Can one say that apparently, the pKa values are, e.g., 2 and 8 while microscopically they are, e.g., 4.5 and 4.6?\\


==> 081-bcx-cosmo-pro.tex <==
\newpage

\section*{Modeling protocol}

\subsubsection*{WT Structure Preparation}
Download enzyme-substrate complex structure 1BCX and inhibited enzyme structure 1BVV.
Use \verb+set retain_order, 0+ option in PyMOL.
In substrate of 1BCX, modify XYP 502 O2B (= -F in inhibitor) to -OH, remove oxygen XYP 502 O4A and ``Fix H'' on carbon XYP 502 C1B, select and copy substrate molecule to new object and save as \verb+sub-es-noh.pdb+.
In substrate of 1BVV, change DFX 502 F2 to -OH, remove bond between DFX 502 C1 and GLU 78 OE2 and ``Fix H'' on DFX 402 C1, select and copy substrate molecule to new object and save as \verb+sub-ge-noh.pdb+.
The atoms of the two substrate structures \verb+sub-es-noh.pdb+ and \verb+sub-ge-noh.pdb+ are synchronized and can be interpolated without further modification.\\
Load \verb+sub-es-noh.pdb+, replace equatorial hydrogen XYP 502 H03 by oxygen, attach benzyl group to newly introduced oxygen XYP 502 O02 and remove possibly remaining hydrogen XYP 502 H03 from newly introduced oxygen.
Attach nitro-group -NO$_2$ to benzyl group and model in PyMOL to remove unphysical distances between atoms of active site and substrate ONP group.
Select and copy only ONP including newly introduced oxygen XYP 502 O02 to new object and save as \verb+onp.pdb+.
Check that axial hydrogen XYP 502 H02 is remaining on XYP 502 C1B.
The atoms of the two substrates including hydrogen on nucleophilic carbon are synchronized and can be interpolated without further modification.\\ 
% Optimization of waters
Load structure 1BVV and select residues N35, Y65, Y80, R112, Q127, W129 and E172 and two catalytic waters HOH218 and HOH237, copy selection to new object and save as \verb+as-ge.pdb+.
Combine \verb+as-ge.pdb+, \verb+sub-ge-noh.pdb+ and \verb+onp.pdb+ to \verb+as-sub-ge-noh-onp.pdb+.
Load \verb+as-sub-ge-noh-onp.pdb+ and locally optimize HOH218 in PyMOL to avoid bond formation between HOH218 and ONP group (or other units) when opening in Avogadro (prevents initialization of force field).
Save HOH218 as \verb+hoh218.pdb+ and replace HOH218 coordinates in \verb+as-sub-ge-noh-onp.pdb+ by newly saved coordinates.\\
% Optimization of ONP group
Open \verb+as-sub-ge-noh-onp.pdb+ in PyMOL, remove superfluous hydrogen XYP 502 H03 and save as \verb+as-sub-ge-noh-onp.pdb+ (overwrite previous version).
Open \verb+as-sub-ge-noh-onp.pdb+ in Avogadro, select ONP group and fix constraints.
Optimize locally ONP group and save as \verb+as-sub-ge-noh-onp-opt.pdb+ (XYP is renamed to LIG by Avogadro).
Open \verb+as-sub-ge-noh-onp-opt.pdb+ in PyMOL, select ONP group and save as \verb+onp-opt.pdb+.\\
% Adding hydrogens to substrate
Load \verb+sub-es-noh.pdb+, add hydrogens and save as \verb+sub-es-h.pdb+.
Load \verb+sub-ge-noh.pdb+, add hydrogens and save as \verb+sub-ge-h.pdb+.
Combine \verb+sub-es-h.pdb+ and \verb+onp-opt.pdb+ to \verb+sub-es-h-onp-opt.pdb+, remove hydrogen XYP 502 H03.
Combine \verb+sub-ge-h.pdb+ and \verb+onp-opt.pdb+ to \verb+sub-ge-h-onp-opt.pdb+, remove superfluous hydrogen XYP 502 H02.
The protonated substrate including the ONP group can be interpolated (the ONP group does not change), the hydrogen on the nucleophilic carbon changes from equatorial to axial.\\
% Addition of transfering proton
Load \verb+1bvv.pdb+ and modify GLU 172 O02 to carry hydrogen.
Select newly introduced hydrogen GLU 172 H01, copy to new object and save as \verb+h-es.pdb+.
Load \verb+sub-ge-h-onp-opt.pdb+ and ``Fix H'' on LIG 3 O.
Load \verb+h-es.pdb+ and orient newly introduced hydrogen LIG 3 H01 towards GLU 172 H01 for reasonble interpolation path.
Select newly introduced hydrogen Lig 3 H01, copy to new object and save as \verb+h-ge.pdb+.\\
% Correct HOH218
Copy \verb+1bvv.pdb+ to \verb+ge-noh-ini.pdb+, discard all non-\verb+ATOM+ and -\verb+HETATM+ records and replace HOH218 coordinates with coordinates from \verb+hoh218.pdb+.
% Add hydrogens to structure
Load \verb+ge-noh-ini.pdb+ in PyMOL, ``Add H'' and save as \verb+ge-h-ini.pdb+.  
% Introduce substrate to protonated structure
Replace substrate records by \verb+sub-ge-h-onp-opt.pdb+ records.
Append \verb+h-ge.pdb+ to \verb+ge-h-ini.pdb+.
Copy \verb+ge-h-ini.pdb+ to \verb+es-h-ini.pdb+, replace substrate records by \verb+sub-es-h-onp-opt.pdb+ records and append \verb+h-es.pdb+.
% Making N-terminal positive
Load \verb+es-h-ini.pdb+ and use ``Charge +1'' on N-terminal nitrogen to generate proton, select newly generated proton ALA 1 H05, copy to new object and save as \verb+h-ala.pdb+.
Insert \verb+h-ala.pdb+ record at appropriate position in \verb+es-h-ini.pdb+ and \verb+ge-h-ini.pdb+.
Substrate in enzyme-substrate complex can be interpolated to bound substrate in glycosyl-enzyme.

\subsubsection*{Preparation of WT interpolation 1}
From both \verb+es-onp-opt-pm6-<GNORM>-<CUTOFF>.pdb+ and \verb+ge-onp-opt-pm6-<GNORM>-<CUTOFF>.pdb+ all \verb+HEADER+ and \verb+TER+ records are discarded.
In PDB files written by MOPAC, substrate is relabeled to \verb+LIG+ and \verb+resi+ is set to \verb+500+.
Interpolation frames are prepared using \verb+intcha.py+ script which computes closed shell overall charge of each frame using MOPAC keyword \verb+charges+.
Charge is determined to be +4 on first, second and last frame, and +2 on third to ninth frame.
To allow setting of optimization flags (\verb&+1& to \verb&+0&) of atoms on reaction coordinate and overwriting of computed charges on atoms, input format is transfered from PDB to MOPAC format by a \verb+1scf+ calculation using \verb+mozyme+ and \verb+cutoff=2+ with the \verb+cha2scf.sh+ script.
The output from the 1SCF calculations is transfered using the \verb+scf2opt.sh+ script which requires the adjustment of the line number variable to control which atoms are constrained (documented within script) and the MOPAC configuration.
%E78 OE2 and C1 (Fig. \ref{fig:substrate_sasm}) of substrate are constrained on reaction path.
E78 OE2 and C1 (Fig. \ref{fig:glycosylation_step}) of substrate are constrained on reaction path.
In interpolation frames 3 to 9, charge of C 3140 (PDB ID) is set to +1 with the \verb+flagAtom.sh+ script (also requiring adjustment) which corrects determined overall charge to +4.

\subsubsection*{Preparation of WT interpolation 2: WT ES' opt}
%Use \verb+ge-onp-opt-pm6-<GNORM>-<CUTOFF>.{mop,out,arc,pdb}+ as template for WT ES' (Fig. \ref{fig:calc_path}).
Use \verb+ge-onp-opt-pm6-<GNORM>-<CUTOFF>.{mop,out,arc,pdb}+ as template for WT ES' (Fig. \ref{fig:calc_path_wt}).
Use \verb+sub-es-h-onp-opt.pdb+ as template for substrate.
Copy \verb+ge-onp-opt-pm6-<GNORM>-<CUTOFF>.pdb+ to \verb+es-onp-ini-pm6-<GNORM>-<CUTOFF>.pdb+, delete GE substrate records (including transfering proton record) and append ES substrate records from \verb+sub-es-h-onp-opt.pdb+.
Eventually, \verb+resn+ and \verb+resi+ records of substrate need to be adjusted.
Also, \verb+resn+ of E78 required adjustement (was written as \verb+UNK+ by MOPAC because of connection to ligand).
Open \verb+es-onp-ini-pm6-<GNORM>-<CUTOFF>.pdb+ in PyMOL, ``Fix H'' on GLU 172 OE2 (easiest by defining charge 0 on oxygen) and model newly introduced hydrogen GLU 172 H01 to be oriented appropriately (to enable linear interpolation with \verb+ge-onp-opt-pm6-<GNORM>-<CUTOFF>.pdb+).
Select and copy newly introduced hydrogen to new object and save as \verb+h-es-ini.pdb+.
Append \verb+h-es-ini.pdb+ to \verb+es-onp-ini-pm6-<GNORM>-<CUTOFF>.pdb+, \verb+es-onp-ini-pm6-<GNORM>-<CUTOFF>.pdb+ and \verb+ge-onp-opt-pm6-<GNORM>-<CUTOFF>.pdb+ can be interpolated, only substrate changes.
Copy \verb+es-onp-ini-pm6-<GNORM>-<CUTOFF>.pdb+ to \verb+es-onp-opt-pm6-<GNORM>-<CUTOFF>.mop+ and carry out optimization.
Using optimized WT ES' structure, steps to prepare interpolation 2 are similar as for WT interpolation 1.

\subsubsection*{Preparation of constrained WT optimization for interpolation 2}
Required: \verb+es-onp-opt-pm6-<GNORM>-<CUTOFF>.mop+ as prepared for unconstrained WT interpolation 2.
%Steps will be 1) to prepare structures with different layers of constrained residues (using the \verb+format_mopac.py+ PyMOL script) and 2) to write a Python script (``Fix'' in Fig. \ref{fig:calc_path}) which is used to define the constraints for the optimizations of Mut GE, Mut ES' (interpolation 4) and Mut ES'' (interpolation 5) using the \verb+check-ca.py+ PyMOL script.
Steps will be 1) to prepare structures with different layers of constrained residues (using the \verb+format_mopac.py+ PyMOL script) and 2) to write a Python script (``Define constraints'' in Fig. \ref{fig:calc_path_wt}) which is used to define the constraints for the optimizations of Mut GE, Mut ES' (interpolation 4) and Mut ES'' (interpolation 5) using the \verb+check-ca.py+ PyMOL script.
Change working directory of PyMOL to location where \verb+es-onp-onp-pm6-<GNORM>-<CUTOFF>.mop+ is.
In PyMOL, use \verb+set retain_order+ (no argument \verb+, 0+ or \verb+, 1+) and \verb+set pdb_retain_ids+ commands to prevent reordering of structure when writing to disk.
In \verb+format_mopac.py+ script, optionally adjust constraint distances array.
Load WT structure and call \verb+PyMOL> run <scripts>/format_mopac.py+, eventually modify output file naming.
Execute \verb+save_mopac_all <REFERENCE>+ to generate the structures \verb+<LABEL>-con-opt-<CONSTRAINT>-ste-ini.pdb+ in MOPAC format with constraint flags set.
Delete and reload structure \verb+es-onp-opt-pm6-<GNORM>-<CUTOFF>.mop+, run \verb+check-ca.py+ script to generate script \verb+fix-<LABEL>-<CONSTRAINT>.py+ (required for preparation of input files for constrained optimization of mutants).
Execute by call \verb+PyMOL> check_rest_ca_resi <selection>+, script \verb+fix-<LABEL>-<CONSTRAINT>.py+ is written.
Copy structures \verb+<LABEL>-con-opt-<CONSTRAINT>-ste-ini.pdb+ to \verb+<LABEL>-con-opt-<CONSTRAINT>-<GNORM>-<CUTOFF>.mop+ and start optimization of constrained WT ES'.  

\subsubsection*{Preparation of interpolation 3}
\textbf{Mutant fragments.} Positions are selected within 4\AA\ of substrate in both ES and GE structure.
In ES, 17 positions are included, in GE 15, only positions selected in both structures are considered.
In ES and GE, substrate records are renamed from \verb+UNK+ to residue name \verb+LIG+, residue ID 500 and chain A.
All atom name specifiers are reduced to bare element name (interpolation was perturbed from specific atom names).
In GE, E78 is labeled as \verb+UNK+ by MOPAC due to its covalent bond to the substrate.
Atom labels are corrected (copied from ES PDB file).
All \verb+END+ and \verb+CONECT+ records are discarded from back bone sequence and mutant side chain fragments and water fragments.

\subsubsection*{Preparation of mutant fragments interpolation 4}
Residue name records of substrate atoms adjusted to \verb+LIG+, all substrate atom chain identifiers set to chain A and residue ID adjusted to \verb+500+ in \verb+ge-onp-opt-pm6-<GNORM>-<CUTOFF>.pdb+ prior to variant side chain generation and back bone sequencing.
Label of E78 is \verb+UNK+ (from MOPAC optimization) and adjusted to \verb+GLU+.
Change working directory of PyMOL to directory containing \verb+ge-onp-opt-pm6-<GNORM>-<CUTOFF>.pdb+.
Enter \verb+set retain_order, 0+ to protect atom ordering of mutant fragments.
Call \verb+PyMOL> run $PyMOL_SCRIPTS/vsc-ext.py+, and execute \verb+PyMOL> frag 3+.
The \verb+vsc-ext.py+ script is a modification of \verb+vsc.py+ in that it mutates every residue within a specified distance to a reference site (such as the substrate).
Load \verb+ge-onp-opt-pm6-<GNORM>-<CUTOFF>.pdb+, call \verb+PyMOL> run $PyMOL_SCRIPTS/seq_files.py+, and execute \verb+PyMOL> seq 3+.
Using \verb+python avf-bcx.py+ the \verb+seq.sh+ script is generated which assembles the mutant structure files.
The \verb+avf-bcx.py+ script is a modificiation of \verb+avf.py+ in that it generates every single mutant back bone depending on the mutant fragment files it finds in the working directory.\\
The structure \textsc{wt es}' is used as template for the mutants.
The substrate \verb+resn+ and \verb+resi+ records are adjuste similarly to above, the \verb+vsc-ext.py+ script is used to prepare the variant side chains.
Using the \verb+seq_files.py+ script, the back bone structure files are prepared.
It is verified that the substrate from \verb+seq-x500-1.pdb+ can be interpolated with the substrate of an optimized mutant.
The optimization of the stationary points is done by first copying the files \verb+1-res-<MUTANT>-ste-ini.pdb+ to \verb+1-con-scf-<MUTANT>-<LAYER>-pm6-<GNORM>-<CUTOFF>.mop+ and carrying out 1SCF calculations using the \verb+1scf+ keyword.
The output of the 1SCF calculations is used as the input for the optimizations, the \verb+fix-es-onp-opt-pm6-1.0-15-8.0.py+ script is used to fix the atoms.

\subsubsection*{Preparation of ES structures interpolation 5}
\textbf{Note}: The difficulty with this strategy is that the substrate is differently optimized for every mutant \textbf{GE} structure.
Ideally, the substrate is replaced such that for every mutant it is replaced individually in order to preserve the specifically optimized geometry of the mutant, but this would require individual manual modeling of each mutant which is not an option.\\
%Steps: Copy all optimized GE PDB structures, rename to \verb+1-ini+ and discard all \verb+HEADER+ and \verb+TER+ records.
%Rename substrate records to \verb+resn LIG+, \verb+resi 500+ and \verb+chain A+.
%Use \verb+sub-es-h-onp-opt.pdb+ as template for substrate in ES.
%In all \verb+1-ini+ structures, discard substrate
%\begin{lstlisting}
%bash $ for i in 1-ini-*
%> do
%> a=`cat $i|wc -l`
%> m=$((a-`cat sub-es-h-onp-opt.pdb|wc -l`))
%> head -n $m $i > ${i/ini/tmp}
%> done
%\end{lstlisting}
%and append \verb+sub-es-h-onp-opt.pdb+.
%%Proton from E172 is appended to all ES'' initial structures (this is a problem, when the proton indeed would be on the ONP substrate leaving group, as it is supposed to be from the mechanism), copy structure to MOPAC input file.  
%The proton from E172 is now appended to all \textsc{es}'' structures identically which can be a problem if E172 is very differently oriented in different mutants.
%To add the proton, open the mutant ES'' complex \verb+1-con-ini-<MUTANT>-<CONSTRAINT_LAYER>-<METHOD>-<GNORM>-<CUTOFF>.pdb+ in PyMOL and set charge to ``0'' on E172, this will add a proton.
%Select the proton and copy it to a new object, save the object and append the coordinates from the atom to the structure file of the mutant ES'' complex.\\
%\textbf{Strategy 1: No optimization of inserted substrate.} The substrate is too close to Q127 and MOPAC forms a bond between the substrate nitro-group and the side chain of Q127, therefore the overall charge is not consistent (+2 instead of +4 as in the GE structure).\\
%\textbf{Strategy 2: Optimization of inserted substrate with PyMOL sculpting.} Using the following sets of commands, the substrate can be optimized after inserting it.
%\begin{lstlisting}[escapechar=\%]
%%\#%First remove wrong bond
%%\#%Select a1 on substrate and a2 on Q127
%PyMOL> select a1, resi 500 and ID 10
%PyMOL> select a2, resi 127 and ID 1895
%PyMOL> unbond a1, a2
%%\#%Fix enzyme, activate sculpt on object and optimize substrate
%PyMOL> select sub, /1-con-ini-N35F-08-pm6-1.0-15///500/
%PyMOL> cmd.protect('(not sub)')
%PyMOL> cmd.sculpt_activate('1-con-ini-N35F-08-pm6-1.0-15')
%PyMOL> cmd.sculpt_iterate('1-con-ini-N35F-08-pm6-1.0-15', cycles=5000)
%PyMOL> cmd.sculpt_deactivate('1-con-ini-N35F-08-pm6-1.0-15')
%PyMOL> cmd.deprotect()
%\end{lstlisting}
%Extract the substrate together with the transfering proton of E172 to a new file \verb+sub-es-h-h172-onp-opt-2.pdb+ and append it to the ES'' structure file.
%The overall charge is now +4 and no bond is formed between the substrate and Q127.
%The problem when not optimizing is identified as MOZYME forming a bond between the terminal H of the Q127 (H1895) side chain and the nitro group of the substrate (while not forming a bond between the terminal H1895 and the nitrogen atom of the Q127 side chain.\\
%\textbf{Strategy 3: Use WT ES' substrate}. Instead of inserting a default substrate, it appears reasonable to introduce the substrate from the optimized \textsc{es}' structure of the \textsc{wt}.\\
\textbf{Strategy: Use WT ES' substrate}.
It appears reasonable to introduce the substrate from the optimized \textsc{es}' structure of the \textsc{wt} and use this as the starting geometry of the substrate for all mutants.
This approach should work as long as the \textsc{es}' structure is not too different from the optimized mutant structure.
%Substrate is introduced and optimized in PyMOL for each mutant using 3000 \verb+cycles+.
%\textbf{Strategy 3: Preparation of mutant \textsc{es}'' structures}.
Steps: Copy \verb+es-con-opt-10-pm6-1.0-15.arc+ (optimized \textsc{es}' structure) to working directory \verb+opt-const-mut-espp-set-2-pm6-1.0-15+.
Copy files \verb+3-con-opt-<MUTANT>-10-pm6-1.0-15.arc+ to working directory.
Extract substrate atoms from optimized \textsc{wt es}' structure to \verb+sub-wt-con-opt-<CONSTRAINT_LAYER>-esp-1.0-15.mop+.
Copy \textbf{GE} structures to \verb+1-con-opt-<MUTANT>-10-pm6-1.0-15.mop+ and discard substrate records from these newly generated \textbf{ES} structure files:
\begin{lstlisting}[escapechar=\%]
%\#% Discarding substrate from ES'' input.
bash $ for i in 1-con-opt-*
> do
> a=`cat $i|wc -l`
> m=$((a-`cat sub-wt-con-opt-10-esp-1.0-15.mop|wc -l`))
> head -n $m $i > ${i/opt/tmp}
> mv ${i/opt/tmp} $i
> done
\end{lstlisting}
Append substrate in \textsc{es}' state (constraint flags \verb&+0& remain valid from \textsc{ge} structure file).
Rename from \verb+.arc+ to \verb+.mop+ file extension.
Discard all non-keyword lines from input files (remain from \textsc{mopac} output in \verb+.arc+ files).
% (Note: Escape characters around \" required!)
\begin{lstlisting}[escapechar=\%]
%\#% Remove MOPAC header.
bash $ for i in 1-con-opt-*.mop
> tot=`cat $i|wc -l`
> lineFin=`grep -i -n %"%FINAL GEOMETRY%"% $i|cut -d %"%:%"% -f 1`
> tail -n -$((tot-lineFin)) $i > tmp.mop
> mv tmp.mop $i
> done
\end{lstlisting}

\subsubsection*{Preparation of interpolation frames int 5}
The interpolation frames are ideally prepared from \textsc{mopac} \verb+.arc+ files to preserve the constraints and to avoid the need of having to transfer from PDB to \textsc{mopac} input format.
Steps: 1) Copy all \textsc{es}'' and \textsc{ge} \verb+.arc+ files to working directory and find common set (it can happen that different numbers of structures for \textsc{es}'' and \textsc{ge} converge). 2) Delete \textsc{mopac} header from \verb+.arc+ files. 3) Use \verb+int_arc2mop.py+ script for preparation of interpolation files.
\begin{lstlisting}[escapechar=\%]
[machine]user @ working $ for i in 1-con-opt-*arc
> do
> n=${i/1-con-opt-/}
> n=${n/-10-pm6-1.0-15.arc/}
> python int_arc2mop.py $i 3-con-opt-$n-10-pm6-1.0-15.arc $n
> done
\end{lstlisting}
4) Use \verb+fix_reacting_atoms.py+ script to set constraints on atoms in all interpolation files.

%> lineFin=`grep -i -n "FINAL GEOMETRY" $i|cut -d ":" -f 1`
\subsubsection*{Issues in modeling of set 2}
In all of the following, \textit{predicted} charge refers to the overall charge obtained from chemical reasoning and \textit{computed} charge refers to the overall charge computed from the \textsc{mozyme} Lewis structure routine.\\
When mutating all positions within 4\AA\ of the substrate, the following issues are observed.
The possible overall charges are +2 (R112[D,E]), +3 (A115[D,E], R112[F,...]), +4 (A115[F,...]), +5 (A115[K,R]), where A115F[,...] means mutation of neutral to neutral side chains.
The mutants need to be checked for correct \textsc{mozyme} computation of overall charge which is done using the \verb+check-charge.sh+ script.
Observed reasons for differences in computed overall charge and predicted charge are mainly problems in placing a large side chain within the interior.
Mostly observed for prolines but also tyrosine.
In all failed cases involving proline, the local optimization of proline was problematic, however not every proline is problematic and fails.
No attempt to resolve this issue is made, all mutants which exhibit problems due to local side chain optimization are discarded immediately upon recognition.\\
First step of calculation preparation is manually discarding all problematic structures (identified by \verb+HAS COVALENT BONDS+ in \textsc{mopac}).
\begin{lstlisting}[escapechar=\%]
machine @ for i in 3-con-cha-*out
          do if grep -qi 'has covalent bonds' $i
              then
                  m=${i/3-con-cha-/}
                  m=${m/-08-pm6-1.0-15.out/}
                  echo $m
              fi
          done
\end{lstlisting}
In the second step, structures where predicted and computed charges do not agree are discarded.

\subsubsection*{Double mutants structure preparation}
The overall charge can now vary much more and requires special attention.
1) Copy all \verb+frag-*.pdb+- and \verb+seq-*.pdb+-files to \verb+files-res-double/+ directory.
In interpolation procedure 5, the structures are only prepared for the GE species.
2) Use \verb+analyse-barriers.py+ script to calculate the lowest barrier for each position and prepare all pairs of mutants with lowest barriers (the script requires a ``barriers.dat'' file).
The combination mutants are (manually) written into the \verb+avf-bcx-double.py+ script.
3) The \textsc{mopac} files for calculating the overall charge are written.
4) The predicted and computed overall charges are compared using the \verb+check-charge-double.py+ script.
5) Use common \verb+cha2scf.sh+ and \verb+scf2opt.sh+ scripts to prepare input files for optimization.
6) Use \verb+fix-es-onp-opt-pm6-1.0-15-10.0.py+ to set constraints.
7) Start optimizations.

\textbf{Barrier distribution diagram preparation in \textsc{R}}:\\
1) \verb+b2 <- read.table("div/ana-mut-barriers-con-set-2-int-5/barriers.dat", sep=" ")+\\
2) \verb+b3 <- read.table("div/ana-mut-barriers-con-10-set-3-int-5/barriers.dat", sep=" ")+\\
3) \verb+p1 <- hist(subset(b2$V2, b2$V2 < 30), breaks=15, xlim=c(0, 30))+\\
4) \verb+p2 <- hist(subset(b3$V2, b3$V2 < 30), breaks=15)+\\
5) \verb+plot(p1, col=rgb(1,0,0,8/9), main="Barrier distribution",+\\
\verb+xlab="Barrier [kcal/mol]", ylab="Mutant count", xlim=c(0,30))+\\
6) \verb+plot(p2, col=rgb(0,0,1,8/9), add=T)+

